Inform: From Compartmental Models to Stochastic Bounded Counter Machines

Compartmental models are used in epidemiology to capture the evolution of infectious diseases such as COVID-19 in a population by assigning members of it to compartments with labels such as susceptible, infected, and recovered. In a stochastic compartmental model the flow of individuals between compartments is determined probabilistically. We establish that certain stochastic compartment models can be encoded as probabilistic counter machines where the configurations are bounded. Based on the latter, we obtain simple descriptions of the models in the PRISM language. This enables the analysis of such compartmental models via probabilistic model checkers. Finally, we report on experimental results where we analyze results from a Belgian COVID-19 model using a probabilistic model checkers.

==> presentations/macros.tex <==
\newcommand{\smallparagraph}[1]{\smallskip\noindent\textbf{#1}}
\newcommand{\tabitem}{~~\llap{\textbullet}~~}
\makeatletter
\newcommand{\pushright}[1]{\ifmeasuring@#1\else\omit\hfill$\displaystyle#1$\fi\ignorespaces}
\newcommand{\pushleft}[1]{\ifmeasuring@#1\else\omit$\displaystyle#1$\hfill\fi\ignorespaces}
\makeatother

% numbers
\newcommand{\tuple}[1]{\ensuremath{\left\langle #1 \right\rangle}}
\newcommand{\indexof}[2]{\ensuremath{#1_{\scriptscriptstyle #2}}}
\newcommand{\N}{\mathbb{N}}
\newcommand{\fun}[1]{\ensuremath{\mathopen{}\mathclose\bgroup\left(#1\aftergroup\egroup\right)}}
% \newcommand{\condition}[1]{\ensuremath{\mathds{1}_{#1}}}
\newcommand{\condition}[1]{\ensuremath{\1_{#1}}}
\newcommand{\vect}[1]{\ensuremath{\bm{#1}}}
\newcommand{\entrywise}[3]{\ensuremath{\tuple{#1}_{#2 \in [#3]}}}
\newcommand{\images}[1]{\ensuremath{\mathrm{Im}\fun{#1}}}
\newcommand{\diam}[1]{\ensuremath{\mathrm{diam}\fun{#1}}}

% MDPs
\newcommand{\mdp}{\ensuremath{\mathcal{M}}}
\newcommand{\states}{\ensuremath{\mathcal{S}}}
\newcommand{\actions}{\ensuremath{\mathcal{A}}}
\newcommand{\transitions}{\ensuremath{\mathcal{T}}}
%\newcommand{\probtransitions}[1]{\ensuremath{\mathbf{P}}^{\scriptscriptstyle\transitions}\ifthenelse{\equal{#1}{}}{}{_{\scriptscriptstyle#1}}}
\newcommand{\probtransitions}{\ensuremath{\mathbf{P}}} %^{\transitions}}
\newcommand{\rewards}{\ensuremath{\mathcal{R}}}
\newcommand{\labels}{\ensuremath{\ell}}
\newcommand{\atomicprops}{\ensuremath{\mathbf{AP}}}
\newcommand{\sinit}{\ensuremath{s_{\mathit{I}}}}
\newcommand{\mdptuple}{\langle \states, \actions, \probtransitions, \rewards, \labels, \atomicprops, \sinit \rangle}
\newcommand{\mdpspace}{\ensuremath{\mathbb{M}}}
\newcommand{\statesmdptuple}[2]{\ensuremath{ \tuple{#1, \actions, \transitions_{\scriptscriptstyle#1}, \rewards_{\scriptscriptstyle#1}, \labels_{\scriptscriptstyle#1}, \atomicprops, #2} }}
\newcommand{\previousstate}{\ensuremath{\state^{\scriptscriptstyle -1}}}
\newcommand{\previousaction}{\ensuremath{\action^{\scriptscriptstyle -1}}}
\newcommand{\state}{\ensuremath{s}}
\newcommand{\vstate}{\ensuremath{\vs}}
\newcommand{\action}{\ensuremath{a}}
\newcommand{\vaction}{\ensuremath{\va}}
\newcommand{\reward}{\ensuremath{r}}
\newcommand{\labeling}{\ensuremath{l}}
\newcommand{\labelset}[1]{\ensuremath{\mathsf{#1}}}
\newcommand{\actbot}{\ensuremath{\bot}}
\newcommand{\act}[1]{\ensuremath{\mathit{Act}\ifthenelse{\equal{#1}{}}{}{(#1)}}}
\newcommand{\trajectories}[1]{\ensuremath{\mathit{Traj}^{fin}_{ #1 }}}
% \newcommand{\inftrajectories}[1]{\ensuremath{\mathit{Traj}_{#1}}}
\newcommand{\inftrajectories}[1]{\ensuremath{\mathit{Traj}}}
\newcommand{\seq}[2]{\ensuremath{#1_{\scriptscriptstyle 0:#2}}}
\newcommand{\trajectory}{\tau}
\newcommand{\trajectorytuple}[3]{\ensuremath{\tuple{#1_{\scriptscriptstyle 0:#3}, #2_{\scriptscriptstyle 0: #3-1}}}}
\newcommand{\trace}{\ensuremath{\hat{\trajectory}}}
\newcommand{\tracetuple}[5]{\ensuremath{\tuple{#1_{\scriptscriptstyle 0:#5}, #2_{\scriptscriptstyle 0: #5-1}, #3_{\scriptscriptstyle 0:#5 - 1}, #4_{\scriptscriptstyle 0: #5}}}}
\newcommand{\defaulttrace}{\ensuremath{\tracetuple{\state}{\action}{\reward}{\labeling}{T}}}
\newcommand{\traces}[1]{\ensuremath{\mathit{Traces}_{#1}}}
\newcommand{\policy}{\ensuremath{\pi}}
\newcommand{\policies}[1]{\ensuremath{\Pi_{#1}}}
\newcommand{\mpolicies}[1]{\ensuremath{\Pi}}
% \newcommand{\mpolicies}[1]{\ensuremath{\Pi_{#1}^{\textnormal {ml}}}}
\newcommand{\safepolicy}[1]{\ensuremath{\Pi_{#1}^{\textnormal {safe}}}}
\newcommand{\steadystate}[1]{\ensuremath{\xi_{#1}}}
\newcommand{\car}{\ensuremath{\scaleto{\rotatebox[origin=c]{90}{$\circlearrowright$}}{1.4ex}}}
\newcommand{\selfloop}[2]{\ensuremath{#1^{\nobreak\hspace{.065em} \car #2 }}}
\newcommand{\getstates}[1]{\ensuremath{\llbracket #1 \rrbracket}}
\newcommand{\valuessymbol}[2]{\ensuremath{V_{#1}^{#2}}}
\newcommand{\values}[3]{\ensuremath{\valuessymbol{#1}{#2}\fun{#3}}}
\newcommand{\approxvalues}[3]{\ensuremath{\hat{V}_{#1}^{#2}\fun{#3}}}
\newcommand{\episodereturn}[1]{\ensuremath{\mathbf{R}_{#1}}}
\newcommand{\qvaluessymbol}[2]{\ensuremath{Q_{#1}^{#2}}}
\newcommand{\qvalues}[4]{\ensuremath{\qvaluessymbol{#1}{#2}\fun{#3, #4}}}
\newcommand{\objective}{\ensuremath{\Omega}}
\newcommand{\bscc}[2]{\ensuremath{\mathcal{B}^{#1}_{#2}}}
\newcommand{\stationary}[1]{\ensuremath{\xi_{#1}}}
\newcommand{\bisimulation}{\ensuremath{\mathcal{B}}}

% VAE
\newcommand{\encodersymbol}{\ensuremath{Q}}
\newcommand{\encoder}{\ensuremath{\encodersymbol_\encoderparameter}}
\newcommand{\encoderinit}{\ensuremath{\encodersymbol_{\encoderparameter, I}}}
\newcommand{\decodersymbol}{\ensuremath{P}}
\newcommand{\decoder}{\ensuremath{\decodersymbol_\decoderparameter}}
% \newcommand{\latentbeliefspace}{\ensuremath{\mathcal{Q}}}
% \newcommand{\transitiontolatent}{\ensuremath{P^{\scriptscriptstyle \transitions}_{\scalebox{.8}{$\scriptscriptstyle \states, \latentstates$}}}}
% \newcommand{\sreset}{\ensuremath{\state_{\text{reset}}}}
% \newcommand{\actreset}{\ensuremath{\action_{\text{reset}}}}
\newcommand{\latenttransitions}{\ensuremath{\transitions_\theta}}
\newcommand{\encoderparameter}{\ensuremath{\iota}}
\newcommand{\decoderparameter}{\ensuremath{\theta}}
\newcommand{\generative}{\ensuremath{\mathcal{G}}}
\newcommand{\wassersteinparameter}{\ensuremath{\omega}}


% Objectives
\newcommand{\discount}{\ensuremath{\gamma}}
\newcommand{\discountedreturn}[1]{\ensuremath{\mathit{Disc}_{#1}}}
\newcommand{\totalreturn}{\ensuremath{\rewards^{\scriptscriptstyle \infty}}}
\newcommand{\unsafe}{\ensuremath{\mathit{Unsafe}}}
\newcommand{\safe}{\ensuremath{\mathit{Safe}}}
\newcommand{\always}{\ensuremath{\square}}
\newcommand{\eventually}{\ensuremath{\lozenge}}
\newcommand{\ltlnext}{\ensuremath{\circ}}
\newcommand{\policyequiv}{\ensuremath{R}}
\newcommand{\until}[2]{\ensuremath{#1 \, \mathcal{U} \, #2}}

% Probability and information theory
\newcommand{\Prob}{\ensuremath{\displaystyle \mathbb{P}}}
%\newcommand{\Pr}{\ensuremath{\mathrm{Pr}}}
\newcommand{\measurableset}{\ensuremath{\mathcal{X}}}
\newcommand{\varmeasurableset}{\ensuremath{\mathcal{Y}}}
\newcommand{\borel}[1]{\ensuremath{\Sigma\fun{#1}}}
\newcommand{\sample}[2]{\ensuremath{\displaystyle #1 \sim #2}}
%\newcommand{\sampledot}{\ensuremath{\boldsymbol{\cdotp}}}
\newcommand{\sampledot}{\ensuremath{{\cdotp}}}
\newcommand{\expectedsymbol}[1]{\ensuremath{\mathop{\mathbb{E}}\ifthenelse{\equal{#1}{}}{}{_{#1}}}}
\newcommand{\expected}[2]{\ensuremath{\expectedsymbol{#1} \left[ #2 \right]}}
\newcommand{\expectmdp}[3]{\ensuremath{\displaystyle  \E_{#1}^{#2} [ #3 ]}}
\newcommand{\entropy}[1]{\ensuremath{\displaystyle H(#1)}}
\newcommand{\divergencesymbol}{\ensuremath{D}}
\newcommand{\divergence}[2]{\ensuremath{\divergencesymbol\fun{#1, #2}}}
\newcommand{\dklsymbol}{\ensuremath{\divergencesymbol_{{\mathrm{KL}}}}}
\newcommand{\dkl}[2]{\ensuremath{\dklsymbol\fun{#1 \parallel #2}}}
\newcommand{\dtvsymbol}{\ensuremath{d_{{TV}}}}
\newcommand{\dtv}[2]{\ensuremath{\dtvsymbol\fun{#1, #2}}}
\newcommand{\mean}{\ensuremath{\vmu}}
\newcommand{\covar}{\ensuremath{\mSigma}}
\newcommand{\normal}[3]{\ensuremath{\displaystyle \mathcal{N} ( #1; #2, #3 )}}
% \newcommand{\distributions}[1]{\ensuremath{\mathcal{P}\fun{#1}}}
\newcommand{\distributions}[1]{\ensuremath{\Delta\fun{#1}}}
%\newcommand{\support}[1]{\ensuremath{Supp\fun{#1}}}
\newcommand{\mode}[1]{\ensuremath{\textit{mode}\fun{#1}}}
\newcommand{\distortion}{\ensuremath{\mathbf{D}}}
\newcommand{\rate}{\ensuremath{\mathbf{R}}}
\newcommand{\dataentropy}{\ensuremath{\mathbf{H}}}
\newcommand{\elbo}{\ensuremath{\mathrm{ELBO}}}
\newcommand{\error}{\ensuremath{\varepsilon}}
\newcommand{\proberror}{\ensuremath{\delta}}

% Distributions
\newcommand{\logistic}[2]{\ensuremath{\mathrm{Logistic}(#1, #2)}}
\newcommand{\bernoulli}[1]{\ensuremath{\mathrm{Bernoulli}(#1)}}
\newcommand{\categorical}[1]{\ensuremath{\mathrm{Categorical}(#1)}}
\newcommand{\relaxedcategorical}[2]{\ensuremath{\mathrm{RelaxedCategorical}(#1, #2)}}
\newcommand{\relaxedbernoulli}[2]{\ensuremath{\mathrm{RelaxedBernoulli}(#1, #2)}}
\newcommand{\logit}{\ensuremath{{\alpha}}}
\newcommand{\logits}{\ensuremath{\vect{\logit}}}
\newcommand{\temperature}{\ensuremath{\lambda}}

% Wasserstein
\newcommand{\wassersteinsymbol}[1]{\ensuremath{W}_{#1}}
\newcommand{\wassersteindist}[3]{\ensuremath{\wassersteinsymbol{#1}\left( #2, #3 \right)}}
\newcommand{\distance}{\ensuremath{d}}
\newcommand{\logic}{\ensuremath{\mathcal{L}}}
\newcommand{\tightoverset}[2]{%
  \tikz[baseline=(X.base),inner sep=0pt,outer sep=0pt]{%
    \node[inner sep=0pt,outer sep=0pt] (X) {$#2$}; 
    \node[yshift=1.2pt] at (X.north) {$#1$};
}}
\newcommand{\bidistance}{\ensuremath{\tightoverset{\,\scriptstyle\sim}{\distance}}}
\newcommand{\logicbidistance}{\ensuremath{\tilde{\distance}^{\logic}}}
%\newcommand{\functionalexpr}{\ensuremath{\mathcal{F}_{\discount}^{\logic}}}
\newcommand{\functionalexpr}{\ensuremath{\mathcal{F}}}
%\newcommand{\diam}{\ensuremath{\textit{diam}}}
%\newcommand{\couplings}[2]{\ensuremath{\Lambda\fun{#1, #2}}}
\newcommand{\couplings}[2]{\ensuremath{\Lambda(#1, #2)}}
\newcommand{\coupling}{\ensuremath{\lambda}}
\newcommand{\proj}{\ensuremath{\Pi}}
\newcommand{\Lipschf}[1]{\ensuremath{\mathcal{F}_{#1}}}
%\newcommand{\Lipschf}[1]{\ensuremath{\norm{\cdot}_{#1}} \leq 1}
%\newcommand{\tracedistance}{\ensuremath{\hat{\distance}}}
\newcommand{\tracedistance}{\transitiondistance}
\newcommand{\transitiondistance}{\ensuremath{\ensuremath{\vec{\distance}}}}
\newcommand{\waemdp}{W$^2\!$AE-MDP$\,$}
\newcommand{\waemdps}{W$^2\!$AE-MDPs$\,$}
\newcommand{\ncritic}{\ensuremath{m}}

% Deep MDPs
\newcommand{\overbar}[1]{\mkern 1.5mu\overline{\mkern-1.5mu#1\mkern-1.5mu}\mkern 1.5mu}
\newcommand{\overbarit}[1]{\,\overline{\!{#1}}}
\newcommand{\embed}{\ensuremath{\phi}}
\newcommand{\embeda}{\ensuremath{\psi}}
% \newcommand{\latentembeda}{\ensuremath{\overbarit{\embeda}}}
\newcommand{\actionencoder}{\ensuremath{\embed_{\encoderparameter}^{\scriptscriptstyle\actions}}}
% \newcommand{\transitionencoder}{\ensuremath{\vec{\embed}}}
\newcommand{\transitionencoder}{\ensuremath{q}}
\newcommand{\latentmdp}{\ensuremath{\overbarit{\mdp}}}
\newcommand{\latentprobtransitions}{\ensuremath{\overbar{\probtransitions}}}
\newcommand{\latentstates}{\ensuremath{\overbarit{\mathcal{\states}}}}
\newcommand{\latentrewards}{\ensuremath{\overbarit{\rewards}}}
\newcommand{\latentlabels}{\ensuremath{\overbarit{\labels}}}
\newcommand{\latentmdptuple}{\ensuremath{\tuple{\latentstates, \latentactions, \latentprobtransitions, \latentrewards, \latentlabels, \atomicprops, \zinit}}}
\newcommand{\latentstate}{\ensuremath{\overbarit{\state}}}
\newcommand{\zinit}{\ensuremath{\latentstate_I}}
\newcommand{\latentactions}{\ensuremath{\overbarit{\actions}}}
\newcommand{\latentaction}{\ensuremath{\overbarit{\action}}}
\newcommand{\latentvaluessymbol}[2]{\overbarit{\ensuremath{V}}_{#1}^{#2}}
\newcommand{\latentvalues}[3]{\ensuremath{\latentvaluessymbol{#1}{#2}\fun{#3}}}
\newcommand{\latentqvaluessymbol}[2]{\ensuremath{\overbarit{Q}_{#1}^{#2}}}
\newcommand{\latentqvalues}[4]{\ensuremath{\latentqvaluessymbol{#1}{#2}\fun{#3, #4}}}
\newcommand{\latentpolicy}{\ensuremath{\overbar{\policy}}}
\newcommand{\latentpolicies}{\ensuremath{\overbar{\Pi}}}
% \newcommand{\latentmpolicies}{\ensuremath{\overbar{\Pi}^{\textnormal {ml}}}}
\newcommand{\latentmpolicies}{\ensuremath{\overbar{\Pi}}}
\newcommand{\localtransitionloss}[1]{L_{\probtransitions}^{#1}}
\newcommand{\localrewardloss}[1]{L_{\rewards}^{#1}}
\newcommand{\localtransitionlossupper}[1]{\dot{L}_{\probtransitions}^{#1}}
\newcommand{\localrewardlossupper}[1]{\dot{L}_{\rewards}^{#1}}
\newcommand{\localtransitionlossapprox}[1]{\hat{L}_{\probtransitions}^{#1}}
\newcommand{\localrewardlossapprox}[1]{\hat{L}_{\rewards}^{#1}}
\newcommand{\KV}{\ensuremath{K_{\latentvaluessymbol{}{}}}}
\newcommand{\KR}[1]{\ensuremath{\ifthenelse{\equal{#1}{}}{K_{\latentrewards}}{K_{\latentrewards}^{#1}}}}
\newcommand{\KP}[1]{\ensuremath{\ifthenelse{\equal{#1}{}}{K_{\latentprobtransitions}}{K_{\latentprobtransitions}^{#1}}}}
\newcommand{\Rmax}[1]{\ensuremath{\ifthenelse{\equal{#1}{}}{|\latentrewards^\star|}{|\latentrewards_{#1}^{\star}|}}}
\newcommand{\stationarydecoder}{{\stationary{\decoderparameter}}}
\newcommand{\latentstationaryprior}{{\bar{\xi}_{\latentpolicy_{\decoderparameter}}}}
\newcommand{\norm}[1]{\ensuremath{\left\| #1 \right\|}}
\newcommand{\gradient}{\ensuremath{\nabla}}
\newcommand{\latentvariables}{\ensuremath{\mathcal{Z}}}
\newcommand{\latentvariable}{\ensuremath{z}}
% \newcommand{\originaltolatentstationary}[1]{{\latentprobtransitions_{\embed_{\encoderparameter}\stationary{\ifthenelse{\equal{#1}{}}{\policy}{#1}}}}}
\newcommand{\originaltolatentstationary}[1]{\ensuremath{\mathcal{T}}}
\newcommand{\varsampledfrom}[3]{\ensuremath{#1}_{{#2}, {#3}}}
\newcommand{\steadystateregularizer}[1]{\ensuremath{\mathcal{W}_{\stationary{#1}}}}
\newcommand{\steadystatenetwork}{\ensuremath{\varphi_{\wassersteinparameter}^{\stationary{}}}}
% \newcommand{\steadystatenetwork}{\ensuremath{f_{\wassersteinparameter}}}
\newcommand{\transitionlossnetwork}{\ensuremath{\varphi_{\wassersteinparameter}^{\probtransitions}}}
% \newcommand{\transitionlossnetwork}{\ensuremath{\varphi_{\wassersteinparameter}}}

% Experience replay
\newcommand{\replaybuffer}{\ensuremath{\mathcal{D}}}
\newcommand{\experience}{\ensuremath{\eta}}
\newcommand{\loss}{\ensuremath{L}}

% Epidemics
\newcommand{\aemdp}{\ensuremath{\latentmdp_{\mathsf{AE}}}}
\newcommand{\cm}{\ensuremath{\mdp_{\mathsf{CM}}}}
\newcommand{\ibm}{\ensuremath{\mdp_{\mathsf{IBM}}}}
\newcommand{\cmtoae}{\ensuremath{\embed_{\scriptscriptstyle\mathsf{CM}\to\mathsf{AE}}}}
\newcommand{\ibmtocm}{\ensuremath{\embed_{\scriptscriptstyle\mathsf{IBM}\to\mathsf{CM}}}}
\newcommand{\ibmtoae}{\ensuremath{\embed_{\scriptscriptstyle\mathsf{IBM}\to\mathsf{AE}}}}
\newcommand{\cmpolicy}{\ensuremath{\policy_{\mathsf{CM}}}}

==> tables/ModestUltimate.tex <==
\begin{table}[]
    \centering
    \caption{Performance of Modest for large populations. Modest was run for the popinc properties in increasingle larger populations in a \emph{start of an epidemic} situation. We ran Modest with the max run lenght set to $0$ and seed $997$.}
    \begin{tabular}{|c|c|c|}
        \hline
         population & result &Modest simulation time \\
        \hline
     (10, 1, 1, 1) & 0.9961538461538462 & 6.1s  \\
     (20, 1, 1, 1) & 0.993 & 9.3s  \\
     (40, 1, 1, 1) & 0.993 & 11.7s  \\
     (80, 1, 1, 1) & 0.9971428571428571 & 12.1s  \\
     (160, 1, 1, 1) & 0.9936842105263158 & 25.2s  \\
     (320, 1, 1, 1) & 0.9983606557377049 & 27.7s  \\
     (640, 1, 1, 1) & 0.9952380952380953 & 68.1s  \\
     (1280, 1, 1, 1) & 1 & 74.7s  \\
     (2560, 1, 1, 1) & 0.9944444444444445 & 257.1s  \\
     (5120, 1, 1, 1) & 0.9944444444444445 & 504.0s  \\
     (10240, 1, 1, 1) & 0.9983606557377049 & 689.8s  \\
     (20480, 1, 1, 1) & 0.9952380952380953 & 1869.1s  \\
     (40960, 1, 1, 1) & 0.9983606557377049 & 2774.2s  \\
     (81920, 1, 1, 1) & 0.9971428571428571 & 6420.6s  \\
     (163840, 1, 1, 1) & 1 & 8882.6s  \\
     (327680, 1, 1, 1) & 0.9952380952380953 & 29609.8s  \\
     (0, 1, 1, 1) &  & s  \\
     (0, 1, 1, 1) &  & s  \\
     (0, 1, 1, 1) &  & s  \\
     (0, 1, 1, 1) &  & s  \\

         \hline
    \end{tabular}
    \label{tab:popincultimate}
\end{table}
